Representation results and error estimates for differential games with applications using neural networks

We study deterministic optimal control problems for differential games with finite horizon. We propose new approximations of the strategies in feedback form, and show error estimates and a convergence result of the value in some weak sense for one of the formulations. This result applies in particular to neural networks approximations. This work follows some ideas introduced in Bokanowski, Prost and Warin (PDEA, 2023) for deterministic optimal control problems, yet with a simplified approach for the error estimates, which allows to consider a global optimization scheme instead of a time-marching scheme. We also give a new approximation result between the continuous and the semi-discrete optimal control value in the game setting, improving the classical convergence order under some assumptions on the dynamical system. Numerical examples are performed on elementary academic problems related to backward reachability, with exact analytic solutions given, as well as a two-player game in presence of state constraints. We use stochastic gradient type algorithms in order to deal with the min-max problem.

==> app3.tex <==
\section{Min-max algorithms [file \texttt{app3.tex}]}\label{app:minmax-algo}
%-------------------------------------------------
\olivier{On adaptera en fonction de ce qui sera utilisé dans la partie num...}

Our typical problem is to deal with $\min\limits_{x}\max\limits_{y}\E \bigg[ J(A(x,Z),B(y,Z),Z)\bigg]$ \red{where $Z$ is a random variable }
over a set of parameters $x\in \R^{n_A}$, $y\in\R^{n_B}$, for given functions $A(x,z)$ and $B(y,z)$ (such as neural networks \red{and in this case we note $A^{\theta_A}$  and $B^{\theta_B}$ to emphasize the fact  that the neural networks depend on some parameters $\theta$ that will be optimized.}),
and for a given function $J(a,b,z)$. 
We recall some stochastic gradient method to deal with some nonconvex - nonconcave problem of the form
\begin{align*}
  %\E\bigg[\min_{x} \max_{y} Q(x,y,Z)\bigg]
  \min_{x} \max_{y}\E\big[ Q(x,y,Z)\big]
\end{align*}
%where $z$ is a noise.\\
where $Z$ is a random variable. At each step $i$, we consider i.i.d. $(z^i_k)_{k=1,\dots,M}$ with same law as $Z$
($z^i_k\sim Z$), and 
\begin{align*}
  f(x,y,z^i) := \frac{1}{M} \sum_{k=1}^M Q(x,y,z^i_k)
\end{align*}
%where $z_i \sim Z$.\\
Algorithm to solve the problem (the first three are for convex-concave problem, while the last one is {\em a priori} 
for more general functionals) :
\begin{itemize}
  \item {\bf SGDA } (\cite{lei2021stability})\\ 
    $(\eta_i)_{i \ge 0}$ a sequence of positive step size:
    \begin{align*}
     x^{i+1} = & x^i -  \eta_i  \nabla_x f(x^i,y^i,z^i) \\
     y^{i+1} = & y^i + \eta_i \nabla_y f(x^i,y^i,z^i)
    \end{align*}
  \item {\bf AGDA} (\cite{lei2021stability})
   $(\eta_{x,i}, \eta_{y,i})_{i \ge 0}$ a sequence of positive step size:
    \begin{align*}
     x^{i+1} = & x^i -  \eta_{x,i}  \nabla_x f(x^i,y^i,z^i_x) \\
     y^{i+1} = & y^i + \eta_{y,i} \nabla_y f(x^{i+1},y^i,z^i_y)
    \end{align*}
    Notice that the noise is different for the two equations.
    \item { $\bf \gamma-GDA$} extension of \cite{jin2020local} in stochastic case. With $\gamma >1$
    $(\eta_i)_{i \ge 0}$ a sequence of positive step size:
    \begin{align*}
     x^{i+1} = & x^i -  \frac{\eta_i}{\gamma}  \nabla_x f(x^i,y^i,z^i) \\
     y^{i+1} = & y^i + \eta_i \nabla_y f(x^i,y^i,z^i)
    \end{align*}
    \item {\bf Potential reduction I} \cite{razaviyayn2020nonconvex}, \cite{jin2020local} \\
    Extension to stochastic case with $(\eta_i)_{i \ge 0}$ a sequence of positive step size.
    \begin{align}
    y^{i+1} = & \argmax_{ y} f(x^i,y, z) \\ 
    x^{i+1} = & x^i -  \eta_i \nabla_x f(x^i,y^i,z^i) 
    \end{align}
    To get a reachable algorithm, we propose 2 versions, {\bf POTE} and {\bf POTEB}:
    \begin{itemize}
      \item {\bf POTE: Version with alternate directions}
    $(\rho_{i,k})_k$  a sequence, $q\geq 1$,
    with $\rho_{i,0}= \rho$, $w^{i,k} \sim z$, $z^i \sim z$:
        %\blue{\olivier{ok comme ca ?} \red{Yes}
        \begin{subequations}
    \begin{align}
      y^{i,0}= & y^i \\
      y^{i,k+1} = & y^{i,k} + \rho_{i,k} \nabla_y f(x^i,y^{i,k},w^{i,k}) , \quad k=0,\dots, q-1 \\ 
    y^{i+1} = & y^{i,q} \\
    x^{i+1} = & x^i -  \eta_i \nabla_x f(x^i,y^{i+1},z^i)
    \end{align}
        \end{subequations}
       %}
\item {\bf POTEB: gradient method on $f(x, \argmax_{y} f(x,y))$.}
    Let $(\rho_{i,k})_k$  a sequence with $\rho_{i,0}= \rho$, $w^{i,k} \sim Z$, $q\geq 1$,
    and let $\phi(x,y)=\phi(x, y, (w^{k})_{k=0,\dots,q-1} , (\rho_{k})_{k=0,\dots,q-1} )$ be such that
    \beno
    y^{0} & = & y \\
    y^{k+1} & = & y^{k} + \rho_{k} \nabla_y f(x,y^{k},w^{k}) , \quad  k=0,\dots,q-1 \\ 
        \phi(x, y)  & = &  (f(x,y^{q}), y^q).
    \eeno
    Then  $f(x,\arg\max_y f(x,y))\simeq  \phi_1(x,y)$ and we do a gradient method in $x$
    \begin{subequations}
     \begin{align}
       x^{i+1}  = &  x^i -  \eta_i \nabla_x \phi_1\big(x^i, y^i,  (w^{i,k})_{k=0,\dots,q-1}, (\rho_{i,k})_{k=0,\dots,q-1}\big) \\ 
       y^{i+1}  = &  \phi_2\big(x^i, y^i, (w^{i,k})_{k=0,\dots,q-1}, (\rho_{i,k})_{k=0,\dots,q-1}\big) \\ 
    \end{align}
    \end{subequations}
  

\end{itemize}
\end{itemize}

In all experiments, we use ADAM \cite{kingma2014adam},
except for Potential reduction one where we use either ADM optimization 
or a classical descent algorithm with a linear reduction of the learning rate SG during the iteration to 1e-5.

Result on rotation test case.
Run 10 times with 10 external iteration $num\_epoch\_ext =10$
\begin{table}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
       & SGDA & AGDA & $\gamma-$GDA & POTENTIAL ADAM &  POTENTIAL SG \\
        Nb success  & 5 &  8 & 2 & 10 & 2
    \end{tabular}
    \caption{Number of success of 10 runs}
    \label{tab:my_label}
\end{table}

% Potential other algorithm to test: NO for non convex, concave
% \begin{itemize}
%     \item \cite{zhang2020single}. To avoid ascillation of SGDA algorithm. To generalize for stochatic gradient with nose $z$. For $p>0$
%     Introduce 
%     \begin{align*}
%     K(x,w,y)= f(x,y) + \frac{p}{2} ||x-w||^2
%     \end{align*}
%      $(\eta_{x,i}, \eta_{y,i})_{i \ge 0}$ a sequence of positive step size, $\beta \in ]0,1]$
%     \begin{align*}
%     x^{i+1} = & x^i -  \eta_{x,i} \nabla_x K(x^i, W^i,y^i,z^i) \\
%     y^{i+1} = & y_i +  \eta_{y,i}  \nabla_y K(x^i, W^i,y^i,z^i) \\
%     w^{i+1} = & w^i +  \beta (x^{i+1}-W^i)       
%     \end{align*}
%     When $\beta =1$, get back SGDA. 
% \end{itemize}



==> ex4-1/sec-num.tex <==
% TODO : check if Time is reverted then $t = T-t$ in the graphs.

\newcommand{\figw}{}
\newcommand{\rdir}{}
\newcommand{\name}{}
\newcommand{\bx}{\overline{x}}{}

\newcommand{\xbmin}{{\underline x}}
\newcommand{\xbmax}{{\overline  x}}
\newcommand{\ybmin}{{\underline y}}
\newcommand{\ybmax}{{\overline  y}}
\newcommand{\epsbmin}{{\underline \epsilon}}
\newcommand{\epsbmax}{{\overline  \epsilon}}

\section{Numerical examples} \label{sec:num}
%---------------------------------------------------

\medskip\noindent
{\bf Feedforward neural networks.}\label{sec:num-nn}
In our approximations we use Feedforward neural networks for the approximation of the feedback control strategies and for the adversarial controls. They are defined as follows : 
$$ ...$$
We use ReLu activation function for all internal activations and some specific activation function for the final layer, 
depending on the example.
When for instance $a=a(x,b)$ and $b=b(x)$ then 
$a$ is approximated by a neural network : $\R^{d+n_B}\conv \R^{n_A}$, assuming $A\subset \R^{n_A}$ and $B\subset \R^{n_B}$,
and $b$ is approximated by a neural network : $\R^{d}\conv \R^{n_B}$.
\xavier{completer ecriture du reseau de neurone (comme dans precedent papier ?)}

All numerical tests are performed using Python 3.10 and Tensorflow. For optimization of the neural network parameters, an SGDA
method is used with ADAM optimizer. In the case of a $\min\limits_{a[\cdot]}\max\limits_{b} Q(a[b],b)$ problem,  
we define $M_{epoch,POTE}$ for a number of internal iterations (optimization of the  parameters of $b$), refereeing to the "POTENTIAL" 
optimization of \cite{...} 
and $M_{epoch}$ for the number of main iterations (optimization of the parameters for $a[]$). 
In the case we consider the equivalent formulation 
$\max\limits_{b} \min\limits_{a[\cdot]} Q(a[b],b)$, then $M_{epoch,POTE}$ is the number of iternal iterations
(thus for the optimization of the $a$ parameters), and $M_{epoch}$ refers to the number of main iterations (for the parameters of $b$).
See Appendix~\ref{app:minmax-algo} for more details.
\xavier{A preciser un peu, on peut referer a l'appendice pour des details}

\subsection{Example 1}\label{sec:num-ex1}
%=---------------------------------------
\olivier{en cours...}
We consider the control problem with control sets $A=B=[-1,1]$ and the following dynamics, for $x\in \R^2$ and $(a,b)\in A\times B$:
$$
   f(x,a,b)= a Rx + c b \frac{x}{\|x\|}
$$
where $c=0.2$, $R=\begin{pmatrix} 0  &  -1\\ 1 & 0\end{pmatrix}$ (rotation matrix), $\|.\|_2$ is the Euclidean norm.
The initial data is
  $$ \varphi(x)= \min(0.5,\max(-0.5,\|x-e\|_2-0.5)
  $$
and obstacle function is
  $$ g(x)= \min(0.5,\max(-0.5,0.75-\|x-q\|_2).
  $$
  with $e=(1,0)$ and $q=(0.75,1)$.
% X0obs=0.75
% Y0obs=1.0
% R-2obs=0.75

(ENCOURS) See Figure~\ref{fig:ex1}
\renewcommand{\figw}{0.50\linewidth}
\begin{figure}[!hbtp]
  \centering
  \renewcommand{\rdir}{ex1/}
  \renewcommand{\name}{g_ex1_fullgrid.eps}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  %\hspace{-4ex}
  %
  \caption{
    (Example 1) Target, no obstacles - for the moment - full grid scheme and analytic 
    $0$-level set.
    %Results obtained with the global scheme
    %Dimension $d=2$, using $N=2,4$ and $8$ time steps (left, middle and right)
    %neural networks of 3 layers and 20 neurons each.
  }
  \label{fig:ex1}
\end{figure}


\subsection{Example 2}\label{sec:num-ex2}
%=---------------------------------------
%2d example where min max = max min (intricate one with analytic sol)

We consider the control problem with control sets $A=B=[-1,1]$ and the following dynamics, for $x\in \R^2$ and $(a,b)\in A\times B$:
%       # res = 2* tf.maximum(-1.0, tf.minimum(1.0, a-2*b))*self.B  + (a+b)*self.C
$$
   f(x,a,b)= \VECT{2 \max(-1,\min(1,a-2b)) \\ a+b},
$$
the terminal value given by
$$
  \varphi(x)= \min(0.5,\max(-0.5, \|x\|_\infty-1)).
$$
In this case we found an analytical formula for the value (see Appendix~\ref{app:vex}).

The parameters are $T=0.4$, and we have tested different number of time steps $N=2,4,8$.
The numerical parameters are otherwise as follows: neural networks using ReLu activation function, numbers of (internal) layers and
neurons per layer $(L,n)=(3,20)$.

Results are given in Figure~\ref{fig:ex2}.


\renewcommand{\figw}{0.30\linewidth}
\begin{figure}[!hbtp]
  \centering
  \renewcommand{\rdir}{ex2/2023-12-22-15h44-save-comm-GlobalNNet2ControlsBFolA-D02-N02-NTstep00-NEXT0100--o20-B1000/}
  \renewcommand{\name}{show__lev_G2BA_D2_Nit2_TStep0_Arelu_Neu20_Lay3_num_epochExt100_Order20_Batch1000_POTE10_ADAM_io0100.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  \hspace{-4ex}
  %
  \renewcommand{\rdir}{ex2/2023-12-22-15h48-save-comm-GlobalNNet2ControlsBFolA-D02-N04-NTstep00-NEXT0100--o20-B1000/}
  \renewcommand{\name}{show__lev_G2BA_D2_Nit4_TStep0_Arelu_Neu20_Lay3_num_epochExt100_Order20_Batch1000_POTE10_ADAM_io0100.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  \hspace{-4ex}
  %
  \renewcommand{\rdir}{ex2/2023-12-22-15h50-save-comm-GlobalNNet2ControlsBFolA-D02-N08-NTstep00-NEXT0100--o20-B1000/}
  \renewcommand{\name}{show__lev_G2BA_D2_Nit8_TStep0_Arelu_Neu20_Lay3_num_epochExt100_Order20_Batch1000_POTE10_ADAM_io0100.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  \hspace{-4ex}
  %
  \caption{
    (Example 2)
    Results obtained with the global scheme
    Dimension $d=2$, using $N=2,4$ and $8$ time steps (left, middle and right)
    neural networks of 3 layers and 20 neurons each.
  }
  \label{fig:ex2}
\end{figure}




\subsection{Example 3}\label{sec:num-ex3}
%---------------------------------------
%2d example where min max $\neq$  max min (intricate one with analytic sol for both min max or max min)

In this example the dynamics is given by 
$$
   f(x,a,b)= \VECT{2 \max(-1,\min(1,|a-b|)) \\ a+b},
$$
with same terminal value $\varphi$ as in the previous example.
An analytical formula for the value is provided in Appendix~\ref{app:vex}.

For the numerical tests, we use the parameter $T=0.4$ and $N=4$ time steps.
The numerical parameters are otherwise as follows: neural networks using ReLu activation function, numbers of (internal) layers and
neurons per layer $(L,n)=(3,20)$.

Results are given in Figure~\ref{fig:ex3}.

\begin{figure}[!hbtp]
  \centering
%show__lev_G2BA_D2_Nit4_TStep0_Arelu_Neu20_Lay3_num_epochExt1000_Order20_Batch1000_POTE10_ADAM_io0700.png
%show__lev_G2BA_D2_Nit4_TStep0_Arelu_Neu20_Lay3_num_epochExt1000_Order20_Batch8000_POTE10_ADAM_io0350.png
%show__lev_G2BA_D2_Nit8_TStep0_Arelu_Neu20_Lay3_num_epochExt100_Order20_Batch1000_POTE10_ADAM_io0000.png
%work__lev_G2BA_D2_Nit16_TStep0_Arelu_Neu20_Lay3_num_epochExt500_Order20_Batch2000_POTE10_ADAM_io0440.png
%work__lev_G2BA_D2_Nit4_TStep0_Arelu_Neu20_Lay3_num_epochExt1000_Order20_Batch2000_POTE10_ADAM_io0000.png
%
%  show__lev_G2BA_D2_Nit8_TStep0_Arelu_Neu20_Lay3_num_epochExt100_Order20_Batch1000_POTE10_ADAM_io0000.png
%  show__lev_G2BA_D2_Nit4_TStep0_Arelu_Neu20_Lay3_num_epochExt1000_Order20_Batch1000_POTE10_ADAM_io0700.png
%  show__lev_G2BA_D2_Nit4_TStep0_Arelu_Neu20_Lay3_num_epochExt1000_Order20_Batch8000_POTE10_ADAM_io0350.png
  %
  \renewcommand{\figw}{0.30\linewidth}
  \renewcommand{\rdir}{ex3/}
  \renewcommand{\name}{show__lev_G2BA_D2_Nit8_TStep0_Arelu_Neu20_Lay3_num_epochExt100_Order20_Batch1000_POTE10_ADAM_io0000.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  \hspace{-4ex}
  %
  \renewcommand{\name}{show__lev_G2BA_D2_Nit4_TStep0_Arelu_Neu20_Lay3_num_epochExt1000_Order20_Batch1000_POTE10_ADAM_io0700.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  \hspace{-4ex}
  %
  \renewcommand{\name}{show__lev_G2BA_D2_Nit4_TStep0_Arelu_Neu20_Lay3_num_epochExt1000_Order20_Batch8000_POTE10_ADAM_io0350.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  \hspace{-4ex}
  %
  \caption{
    (Example 3)
    Results obtained with the global scheme
    (dimension $d=2$), using $N=4$, left: terminal data, middle: $\min-\max$ and right: $\max-\min$,
    neural networks of 3 layers and 20 neurons each.
  }
  \label{fig:ex3}
\end{figure}



\subsection{Example 4}\label{sec:num-ex4}
%---------------------------------------
We consider now a two-player game, where the first player is $X_1=(x_1,x_2)$ with dynamics given by
\beno
 \left\{\barr{l}
  \dot x_1(t) = V_1 \cos(a(t))\\
  \dot x_2(t) = V_1 \sin(a(t))
 \earr\right.
\eeno
with a control which is the "direction" $a(t)\in A:=[-\pi,\pi]$,
and the second player is modelized similarly by $X_2=(x_3,x_4)$ with dynamics
\beno
 \left\{\barr{l}
  \dot x_3(t) = V_2 \cos(b(t))\\
  \dot x_4(t) = V_2 \sin(b(t))
 \earr\right.
\eeno
with an adverse control $b(t)\in B:=[-\pi,\pi]$.
In the numerical example we consider horizon parameter and velocities as follows
$$
  \mbox{$T=4$, $V_1=1$, $V_2=0.7$.}
$$
In this example, $x\in \R^4$ and the global dynamics is therefore given by 
$$
  f(x,a,b):=(V_1\cos(a),V_1\sin(a),V_2\cos(b),V_2\sin(b)).
$$
This example is chosen a little more complex than the previous examples in the sense that we will not have an analytic solution, it is higher dimensional,
but a reference solution can still be obtained by using a classical full grid approach with a finite difference scheme.
Also it is a "commutative" example in the sense that the controls can be separated in the dynamics since we have
\beno
  f(x,a,b) & = & V_1(\cos(a),\sin(a),0,0) + V_2(0,0,\cos(b),\sin(b))  \\
    & = & f_1(x,a) + f_2(x,b).
\eeno


The first player, starting at a given point $(x_1,x_2)\in \R^2$ aims to reach a target $\cC=B_2(x_A,r_A)$ (the Euclidian ball centered at $x_A$ and of radius $r_A$),
at some time $\tau$ before $T$,
keeping away from the the second player starting at $(x_3,x_4)\in \R^2$ (i.e. $\|X_1(t)-X_2(t)\|_2\geq R_0$, for a given threshold $R_0 > 0$) 
for all $t\in[0,\tau]$ whatever the adverse control can be,
staying also in a given domain $X_1\in \cK_1=\mO\backslash int(\cO)$ of $\R^2$, where $\mO:=[\xbmin,\xbmax]\times [\ybmin,\ybmax]$ 
and where $\cO$ is a small square obstacle which is defined here by
$\cO:=B_\infty(x_B,r_B)=\{x\in\R^2,\ \|x-x_B\|_\infty\leq r_B\}$ (so $X_1(t) \in \cK_1$ for all $t\in [0,\tau]$).




Following \cite{bok-for-zid-2010-2},
the problem is a reachability problem with state constraints, which can be reformulated as follows.
We consider the value $v_0(x)$ as in \eqref{eq:v0}, which we recall 
$$
  v_0(x)= \inf_{\ma[.]\in \mG_{(0,T)}} \sup_{b\in \cB_{T}} \ \ 
    \max\bigg( \varphi\big(y_{0,x}^{\ma[b],b}(T)\big), \ \max_{\mt\in (0,T)} g\big(y_{0,x}^{\ma[b],b}(\mt)\big) \bigg)
$$
where the obstacle function $g$ and the terminal cost $\varphi$ are now defined.
We consider truncation values $\epsbmax=0.2$, $\epsbmin=-0.2$.
For $x=(x_1,x_2,x_3,x_4)$, let the terminal cost be defined by
$$
  %\varphi(x) := \max(\epsbmin, \min(\epsbmax, \|(x_1,x_2)-x_A\|_2 - r_A))
  \varphi(x) :=  \|(x_1,x_2)-x_A\|_2 - r_A
$$
(so that $\varphi(x)\leq 0$ $\equivalent$ $(x_1,x_2)\in B_2(x_A,r_A)$).
For the obstacle part, let
$$
  g(x):=\min(g_0((x_1,x_2)),g_d((x_1,x_2)),g_a(x))
$$ 
where
$g_0(.)$ is a level set function to encode the obstacle $B_\infty(x_B,r_B)$:
$$
  %g_0(x):=\max(\epsbmin,\min(\epsbmax, r_B-\|(x_1,x_2)-x_B\|_\infty))
  g_0(x):= r_B-\|(x_1,x_2)-x_B\|_\infty
$$
(so that $g_0(x)\leq 0$ $\equivalent$ $x\in \R^2\backslash B_\infty(x_B,r_B)$),
\COMMENTG{
$g_d(.)$ is a level set function to encode the domain $\mO$
$$
  g_d(x):=\frac{\epsbmax}{\eps_d}\max(x_1-\xbmax,\xbmin-x_1,x_2-\ybmax,\ybmin-x_2),
$$
using a margin parameter $\eps_d:=0.4$, so that 
$g_d(x)\leq 0$ $\equivalent$ $x\in \mO\times \R^2$.
}
Finally $g_a(.)$ is defined by
$$
  %g_a(x):=\max(\epsbmin,\min (\epsbmax,\ R_0- \|(x_1,x_2)-(x_3,x_4)\|_2)),
  g_a(x):=R_0- \|(x_1,x_2)-(x_3,x_4)\|_2,
$$
so that $g_a(x)\leq 0$ $\equivalent$ $\|(x_1,x_2)-(x_3,x_4)\|_2\geq R_0$
(i.e., $g_a(x)$ is a level set function to encode the avoidance of $X_1$ with $X_2$).

For the numerical computations we use also the parameters
%double xB[2]={0.50, 1.50};      //- coordonnees d'un point B (OBSTACLE)
%double rB=0.75;                 //- rayon cible 
$$
  \mbox{$x_A=(3,0)$, $r_A=1$ $\quad$ and $\quad$ $x_B=(0.5,1.5)$, $r_B=0.75$}.
$$
as well as 
$$
  \xbmax=\ybmax:=4.6,\ \xbmin=\xbmin:=-4.6.
$$
(The whole computational domain will be $\cF:=[-8,8]^4$).
and notice then that $v(t,x)=\epsbmax$ whenever $x\notin \cF$).

\MODIFO{
Computations are done with neural networks using $3$ layers of $20$ neurons each,
which corresponds respectively to $(N_a,N_b)=(1044,1004)$ network parameters for each feedback functions $a_k$ and $b_k$ at each time step,
the number of batch points is $N_{batch}=20000$ and the number of SG iterations $N_{epoch}=1000$. Here we observe a numerical convergence
after about $N_{epoch}=500$ iterations, after which small oscillations remain.
}

Results are given in Figure~\ref{fig:ex4-1} ($N=2$, $4$ and $8$ time iterations).
%and Figure~\ref{fig:ex4-2} ($N=8$).
The doted (orange) region corresponds to the points $(x_1,x_2)$ or $\R^2$ such that $v(0,x)\leq 0$, where $x=(x_1,x_2,\bx_3,\bx_4)$
and $(\bx_3,\bx_4)$ has a given value (e.g. $(-2,0)$ in the Figures). This region represent the feasible region, from which it 
is safely possible to reach the target before capture. % and $(3,3)$ in figure \ref{fig:ex4-2}).
The green region represents the target. 
The left figure represents the target (corresponding to the negative region of the value at terminal time).
About $10\%$ of the batch points are also projected in the plane of visualisation.


%\red{
%Time is reverted then $t = T-t$ in the graphs.
%}

%--------------------------------
%- Example 4 - "2a" parameters
%--------------------------------

%% \begin{figure}[!hbtp]
%%   \centering
%%   %
%%   \renewcommand{\figw}{0.30\linewidth}
%%   \renewcommand{\rdir}{ex4/}
%%   %
%%   \hspace{-2cm}
%%   %
%%   %\begin{tabular}{ccc}
%%   \renewcommand{\name}{g_ex4_t6_init.jpg}
%%   \includegraphics[height=\figw,align=c]{\rdir\name}
%%   \hspace{-10ex}
%%   %
%%   \renewcommand{\name}{g_ex4_t6_2a.jpg}
%%   \includegraphics[height=\figw,align=c]{\rdir\name}
%%   \hspace{-10ex}
%%   %
%%   \renewcommand{\name}{g_ex4_t6_2a_traj.jpg}
%%   \includegraphics[height=\figw,align=c]{\rdir\name}
%%   \hspace{-10ex}
%%   % 
%%   \caption{
%%     (Example 4)
%%     \MODIFO{[EXAMPlE 2-a]} cut in plane $(\bx_3,\bx_4)=(-1,0)$ for the adverse starting position.
%%     FD scheme, left: terminal data, middle: ..., right: ... + trajectories of $(x_1(t),x_2(t))$ (black) and $(x_3(t),x_4(t))$ (blue),
%%     (for the adverse control $b(t)$ such that $\dot X_2 = V_2 (X_1-X_2)/\|X_1-X_2\|_2$).
%%   }
%%   \label{fig:ex4}
%% \end{figure}



%--------------------------------
%- Example 4 - "2c" parameters
%--------------------------------
%% \begin{figure}[!hbtp]
%%   \centering
%%   %
%%   \renewcommand{\figw}{0.30\linewidth}
%%   \renewcommand{\rdir}{ex4/}
%%   %
%%   \hspace{-2cm}
%%   %
%%   %\begin{tabular}{ccc}
%%   \renewcommand{\name}{g_ex4_t6_init.jpg}
%%   \includegraphics[height=\figw,align=c]{\rdir\name}
%%   \hspace{-10ex}
%%   %
%%   \renewcommand{\name}{g_ex4_t6_2c.jpg}
%%   \includegraphics[height=\figw,align=c]{\rdir\name}
%%   \hspace{-10ex}
%%   %
%%   \renewcommand{\name}{g_ex4_t6_2c_traj.jpg}
%%   \includegraphics[height=\figw,align=c]{\rdir\name}
%%   \hspace{-10ex}
%%   %\end{tabular}
%%   %
%%   \caption{
%%     (Example 4)
%%     \MODIFO{[EXAMPlE 2-c]} cut in plane $(\bx_3,\bx_4)=(3,3)$ for the adverse starting position.
%%     %\\
%%     %Results obtained with 
%%     %FD scheme (dimension $d=4$), left: terminal data, middle: ..., right: ... + trajectories of $X_1$ (black) and $X_2$ (blue) 
%%     %(for some given adverse control).
%%   }
%%   \label{fig:ex4-2}
%% \end{figure}

%-------------
%- FIG ex4-1
%-------------
\begin{figure}[!hbtp]
  \centering
  %


  %--------------------------------------
  %- N=2
  %--------------------------------------
%fig__surf_G2AB_D4_Nit2_TStep2_Arelu_Neu20_Lay3_num_epochExt200_Order20_Batch20000_POTE20_ADAM_io0000.png
%fig__surf_G2AB_D4_Nit2_TStep2_Arelu_Neu20_Lay3_num_epochExt200_Order20_Batch20000_POTE20_ADAM_io0070.png
%show__lev_G2AB_D4_Nit2_TStep2_Arelu_Neu20_Lay3_num_epochExt200_Order20_Batch20000_POTE20_ADAM_io0070.png
%work__lev_G2AB_D4_Nit2_TStep2_Arelu_Neu20_Lay3_num_epochExt200_Order20_Batch20000_POTE20_ADAM_io0000.png
%work__lev_G2AB_D4_Nit2_TStep2_Arelu_Neu20_Lay3_num_epochExt200_Order20_Batch20000_POTE20_ADAM_io0070.png
  \renewcommand{\figw}{0.30\linewidth}
  \renewcommand{\rdir}{ex4-0/} % N=2 
  \footnotesize{$N=2$}\hspace{-1ex}
  %
  \renewcommand{\name}{show__lev_G2AB_D4_Nit2_TStep2_Arelu_Neu20_Lay3_num_epochExt200_Order20_Batch20000_POTE20_ADAM_io0000.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  %\hspace{-2cm}
  %
  \renewcommand{\name}{show__lev_G2AB_D4_Nit2_TStep2_Arelu_Neu20_Lay3_num_epochExt200_Order20_Batch20000_POTE20_ADAM_io0070.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  %\hspace{-2ex}
  %
  \renewcommand{\name}{fig__surf_G2AB_D4_Nit2_TStep2_Arelu_Neu20_Lay3_num_epochExt200_Order20_Batch20000_POTE20_ADAM_io0070.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}



  %--------------------------------------
  %- N=4
  %--------------------------------------
  \renewcommand{\figw}{0.30\linewidth}
  \renewcommand{\rdir}{ex4-1/} % N=4
  \footnotesize{$N=4$}\hspace{-1ex}
  %
  %\hspace{-2cm}
  %
  \renewcommand{\name}{show__lev_G2AB_D4_Nit4_TStep1_Arelu_Neu20_Lay3_num_epochExt200_Order20_Batch20000_POTE20_ADAM_io0000.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  %\hspace{-10ex}
  % 
  \renewcommand{\name}{show__lev_G2AB_D4_Nit4_TStep1_Arelu_Neu20_Lay3_num_epochExt200_Order20_Batch20000_POTE20_ADAM_io0200.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  %\hspace{-10ex}
  %
  \renewcommand{\name}{fig__surf_G2AB_D4_Nit4_TStep1_Arelu_Neu20_Lay3_num_epochExt200_Order20_Batch20000_POTE20_ADAM_io0200.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  %\hspace{-10ex}
  %
  % 
  
  %--------------------------------------
  %- N=8
  %--------------------------------------
  \renewcommand{\figw}{0.30\linewidth}
  \renewcommand{\rdir}{ex4-2/} % N=8
  \footnotesize{$N=8$}\hspace{-1ex}
  %
  %\hspace{-2cm}
  %
  \renewcommand{\name}{show__lev_G2AB_D4_Nit8_TStep0_Arelu_Neu20_Lay3_num_epochExt200_Order20_Batch20000_POTE20_ADAM_io0000.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  %\hspace{-2cm}
  %
  \renewcommand{\name}{show__lev_G2AB_D4_Nit8_TStep0_Arelu_Neu20_Lay3_num_epochExt200_Order20_Batch20000_POTE20_ADAM_io0200.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  %\hspace{-2ex}
  %
  \renewcommand{\name}{fig__surf_G2AB_D4_Nit8_TStep0_Arelu_Neu20_Lay3_num_epochExt200_Order20_Batch20000_POTE20_ADAM_io0200.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  %\hspace{-2ex}
  %

  \caption{
    (Example 4, $d=4$)
    cut in plane $(\bx_3,\bx_4)=(0,-2)$ for the adverse starting position.
    "Global" scheme with $N=2,4,8$ time iterations, plots of the
    %Comparison of the "Global" scheme with an "exact" FD scheme used for reference,
    %using $N=4$ time iterations.
    $0$-level sets of the terminal value (left) and of the value an initial time (center), surface plot of the value at initial 
    time (right).
  }
  \label{fig:ex4-1}
\end{figure}

%\vspace*{-3cm}

%-------------
%- FIG ex4-2
%-------------
\if{
\begin{figure}[!hbtp]
  \centering
  %
  \renewcommand{\figw}{0.32\linewidth}
  \renewcommand{\rdir}{ex4-2/}
  %
  %\hspace{-2cm}
  %
  \renewcommand{\name}{show__lev_G2AB_D4_Nit8_TStep0_Arelu_Neu20_Lay3_num_epochExt200_Order20_Batch20000_POTE20_ADAM_io0000.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  %\hspace{-2cm}
  %
  \renewcommand{\name}{show__lev_G2AB_D4_Nit8_TStep0_Arelu_Neu20_Lay3_num_epochExt200_Order20_Batch20000_POTE20_ADAM_io0200.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  %\hspace{-2ex}
  %
  \renewcommand{\name}{fig__surf_G2AB_D4_Nit8_TStep0_Arelu_Neu20_Lay3_num_epochExt200_Order20_Batch20000_POTE20_ADAM_io0200.png}
  \includegraphics[height=\figw,align=c]{\rdir\name}
  %\hspace{-2ex}
  %
  % 
  \caption{
    (Example 4, $d=4$)
    cut in plane $(\bx_3,\bx_4)=(0,-2)$ for the adverse starting position.
    "Global" scheme with $N=8$ time iterations.
    %with an "exact" FD scheme used for reference,
    Left: surface plot of the value,
    right: 0-level sets. 
  }
  \label{fig:ex4-2}
\end{figure}
}\fi



\if{

\becolblue

{\bf Example 1.}
We consider in $\R^2$ the two-dimensional dynamics
$$f(x,a,b)= a e_1 + b e_2 \equiv \VECT{a\\b}$$
We look for the stable region under controls $a\in A=[-1,1]$ and uncertainties $b\in[-\frac{1}{2},\frac{1}{2}]$:
$$ \mO^\cK_\infty:=\{ x\in \R^2,\ \exists a[\cdot]\in \mG,\ \forall b(.)\in \cB,\ \forall t\geq 0,\ y_x^{a[b],b}(t)\in \cK\},$$
(where $\mG$ is the set of non-anticipative controls with values in $A$, and $\cB$ is ...)
where $y(t)=y_x^{a,b}(t)$ is the solution of
\beno
    & & \dot y (t) = f(y(t),a(t),b(t)),\quad t\geq 0,\\
    & & y(0)=x.
\eeno
\rd{Is the control depending on $t$ ?
Is it 
\beno
    & & \dot y (t) = f(y(t),a(y(t)),b(y(t))),\quad t\geq 0,\\
    & & y(0)=x.
\eeno
}
\black{{\bf OB:} we will discuss this (As far as I understand : the first allows disconstinuous - only measurable controls and is the correct general math formulation; 
the second formulation assumes Lipschitz feedback functions for well-posedness, 
and is in general the one we use for the code and approximations)}


\fbox{DOMAIN $\mO$ to be removed}

Here the state constraints $\cK$ are composed of a given box (rectangular) domain $\cK_0:=\prod_{i=1}^d [A_i,B_i]$,
and we impose a rectangular obstacle $\cO:=\prod_i]\ma_i,\mb_i[$ so that $\cK:=\cK_0\backslash\cO$. 

The box domain is  modelized by $g_{\cK_0}(x)=\min(\eps_0, \max\limits_i \max(A_i-x_i,x_i-B_i))$
(so that $g_{\cK_0}(x)\leq 0$ $\equivalent$ $x\in \cK_0$), 
and the rectangular obstacle by 
$g_{\cO^\complement}(x)=\min(\eps_0, - \max\limits_i \max(\ma_i-x_i,x_i-\mb_i))$
(so that $g_{\cO}(x)\leq 0$ $\equivalent$ $x\in\cO^\complement$, where 
$\cO^\complement=\R^2\backslash \cO$).
Then we set $g(x)=\max(g_{\cK_0}(x),g_{\cO^\complement}(x))$,
so that $g(x)\leq 0$ $\equivalent$ $x\in \cK:=\cK_0\backslash\cO$.

\begin{rem}
  \black{\bf OB (correctif).} 
  If we do not impose the box constraint (the only condition is to avoid the obstacle $\cO$), then we can take simply 
  $g(x):=g_{\cO^\complement}(x)$.
\end{rem}

\eecol
}\fi


==> sec2-discussion.tex <==
\section{OLD NOTES \texttt{sec2-discussion.tex}}
%--------------------------

\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\bX}{{\bar X}}
\newcommand{\bU}{{\bar U}}

On se concentre sur un probleme à 1 joueur, avec le probleme ideal suivant
\bl{(approximation dans le cas $p=1$):}
$$
  V(x) = \inf_{a\in A} g(x) \vee e^{-\ml h} V(F^a(x)). 
$$
Moralement on approche le problème continu suivant (equation HJB associée):
$$
  \min( \ml v(x) + \max_{a\in A} (-f(x,a) \cdot \nabla v(x)), \ v(x)-g(x)) = 0, \quad x\in \R^d
$$


\medskip\noindent

\blue{
\begin{rem} 
{Cas de $p\geq 1$ (problème de maximum).} 
Une approximation plus précise avec $p$ sous-pas de temps dans l'intervalle $[0,\Dt]$
conduit au problème suivant:
$$
  V(x) = \inf_{a\in A} G^a(x) \vee e^{-\ml \Dt} V(F^a(x)),
$$
avec
$$  G^a(x)=\max_{0\leq k < p}  e^{-\ml k h} g(Y_{k,x}^a) 
$$   
et où $F^a(x)=Y_{p,x}^a$ et $Y_{k,x}^a$ correspond à $k$ itérés de l'application $y\conv F_h(y,a(x))$, partant 
de $y=x$ ($F_h(x,a)$ étant le schéma RK standard avec un pas $h=\dt/p$) :
$$ 
   Y_{k+1,x}^a = F_h(Y_{k,x},a(x)), \quad k\geq 0, \quad Y_{0,x}^a=x.
$$
\end{rem}
}

\centerline{
\fbox{NOTE QUE c'est $a(x)$ qui est utilisé, constant, dans les itérations sur les $Y_{k,x}^a$,
et non pas des $a(Y_{k,x}^a)$}
}

\blue{
\begin{rem} 
Cas d'un problème intégral: 
$$
  v(x) = \inf_{u(.) \in \cU} \int_0^\infty e^{-\ml t} \ell(y_x^u(t),u(t))dt 
$$
Alors le PPD discret, avec $p\geq 1$ sous-pas de temps dans $[0,\Dt]$, peut etre le suivant:
$$
  V(x)= \inf_{a\in A} 
    %\bigg( \frac{1}{p} \sum_{k=0}^{p-1} e^{-\ml k h} \ell(Y_{k,x}^a)  + e^{-\ml \Dt} V(F(x,a)) \bigg)
    \bigg( L(x,a) + e^{-\ml \Dt} V(F(x,a)) \bigg)
$$
avec 
$$ 
    L(x,a)= \frac{1}{p} \sum_{k=0}^{p-1} e^{-\ml k h} \ell(Y_{k,x}^a).
$$
\end{rem}
}


\medskip\noindent
{\bf Algorithme 0.}
Notons $\displaystyle \mG^a(V)(x) : = g(x) \vee  e^{-\ml h} V(F^a(x))$.
Une approche naive serait de considérer
$$ \inf_{V\in \cN} 
 \E\bigg[ \bigg| V(X) -  \inf_{a\in A} \mG^a(V)(X)\bigg|^2 \bigg]
$$
où $\cN$ désigne un espace de fonctions réseaux de neurones dans lequel 
on va chercher à optimiser. On obtient alors un $\hat V$ approché
(avec une erreur donnée $\eta$ pour le probleme de minimisation précédent)
%\rd{Je ne vois même pas comment mettre en oeuvre cette optimisation.}
\blue{(en supposant qu'on sache calculer ou approcher la valeur 
$\inf_{a\in A}\Gamma^a(V)(x)$ pour tout $x$.)}
L'inconvénient de ce type d'approche est que je n'arrive rien à prouver
mathématiquement sur l'erreur $\hat V- V$ en fonction de $\eta$ par exemple,
et cela à cause de la gestion du $"\inf_{a\in A}"$ (qui intervient 
dans $\E[\inf_{a\in A} (...) ]$).
Je cherche à la fois un schema raisonnable et 
à garder une base mathématique pour avoir un ensemble cohérent.
Afin de pouvoir utiliser des techniques similaires à notre précédent travail
(estimation par déformation et changement de variable...)
il faut gérer plutôt une quantité du type 
$$ \inf_{a\in \cA} \E[ \mG^a(V)(X) ] .$$



C'est pourquoi finalement je préfère garder une approche itérative.
Voici deux propositions assez similaires 
(après avoir pas mal tourné en rond) ...
Aussi dans la proposition 2 j'ai essayé de clarifier une manière de coder 
directement $\hV_n(.)$ comme réseau de neurone (Lipschitz) 
plutot que $\ha_n(.)$ (qui est potentiellement discontinu) - comme ce que je voulais faire dans des précédentes discussions.

Pour l'algorithme 1 qui suit je pense qu'on peut avoir une estimation théorique de l'erreur (en suivant 
\cite{bok-pro-war-23}, 
en utilisant des sous-pas de temps, etc..., mais avec des résultats théoriques dont je ne suis pas très satisfait (car besoin de regulariser le controle optimal potentiellement discontinu par des controles plus reguliers...).
Dans la proposition 2 c'est pas clair comment conclure l'estimation, 
mais potentiellement on approche des fonctions Lipschitz par des réseaux de neurones
donc c'est mieux que d'approcher des controles discontinus.

\begin{rem} Il y a aussi une autre information dans les algos ci-dessous, mais pas utilisée, c'est que a priori les $\ha_n$ successifs devrait converger
vers un même $\ha$ optimal.
\end{rem}

\medskip\noindent
{\bf Algorithme 1.}
Dans ce qui suit,  $\hat \cA$ désigne un espace d'approximation pour les contrôles.
On considère une approximation initiale $\hV_0$ (par exemple $\hV_0=g$, la fonction obstacle).
Puis on itère:
\begin{quote}
  $$ \ha_n(.)\in \argmin_{a\in \hat\cA} \E[ \mG^a(\hV_n)(X) ] $$
couplé avec
$$ \hV_{n+1}(x) = \mG^{\ha_n}(\hV_n)(x) $$
\end{quote}
Ce qui signifie que à l'étape $n$ on aura (si $\hV_0=g$) 
$$
  \hV_{n}(x)= J_n(x,\ha) = g(x) \vee e^{-\ml h} g(X^\ha_{1,x}) \vee 
  \cdots \vee e^{-\ml nh} g(X^\ha_{n,x}).
$$
avec les notations (verifier pour les indices...)
$X^a_{k+1,x}:= F(X^a_{k,x}, a_{n-1-k}(X^a_{k,x})) \equiv F^{a_{n-1-k}}(X^a_{k,x})$ for $k\geq 0$ and $X^a_{0,x}=x$,
$a=(a_0,a_1,\dots,a_{n-1})$.

Dans ce procédé on pourrait décider à un moment donné de projeter le résultat
$\hV_n$ sur un réseau de neurones
(ce serait alors une sorte de version hybride...)

\rd{OK c'est clair, c'est pareil que dans l'autre article. On sera limité par le nombre N.\\
On peut aussi faire la version globale !!\\
On fixe  $n$, et on résout avec un seul réseau:
\begin{align}
    \hat a  \in \argmin_{a\in \hat\cA} \E[ J(X,a)]
\end{align}
avec
\begin{align}
J(x,a) = g(x) \vee e^{-\ml h} g(X^a_{1,x}) \vee 
  \cdots \vee e^{-\ml nh} g(X^a_{n,x}).
\end{align}
et
$X^a_{k+1,x}:= F(X^a_{k,x}, a(X^a_{k,x}))$.
Après on fait un calcul pour différent $n$ et on arrête quand $a$ ne bouge plus.
}

\medskip\noindent
{\bf Algorithme 2.}
Dans ce qui suit, $\hat \cN$ désigne un espace d'approximation pour la fonction valeur.
On considère une approximation initiale $\hV_0$ (par exemple $\hV_0=g$, la fonction obstacle.
Puis on itère:
\begin{quote}
  $$ \argmin_{V\in \hat\cN} \E[ \mG^{a_V}(\hV_n)(X) ] $$
  où $a_V (x)=\bar a(x,\nabla V(x))$ est une fonction explicite donnée par l'utilisateur,
  et qui réalise (en lien avec l'EDP continue par ex...)
  $$ \bar a(x,p) = \argmax_{a\in A} (- f(x,a) \cdot p).
  $$
  Ceci est alors couplé avec $\ha_n(x)=\bar a(x,\nabla \hV_n(x))$ et
$$ \hV_{n+1}(x) = \mG^{\ha_n}(\hV_n)(x). $$
\end{quote}
L'intérêt est de gérer des $V$ Lipschitz (on s'attend à ce que $V$ soit Lipschitz) 
qui permettent d'encoder des $a(.)$ discontinus, de manière cohérente
avec le problème considéré.
\rd{Possible is si la fonction explicite est donnée}

\bigskip

\noindent
{\bf Test 1.}
Here is a first test in an LQR infinite horizon context.

Problem : 
$$
  v(x) = \inf_{u(.) \in \cU} \int_0^\infty e^{-\ml t} \ell(y_x^u(t),u(t))dt 
$$
with $\cU = L^\infty((0,\infty),U)$ and $U\subset \R^q$ for some $q\geq 1$.
We consider $U=\R^q$ in order to obtain an analytical solution first. (For numerics we can consider a compact subset 
$U$, see below.)
The dynamics is 
$$
  f(x,u)= Ax + Bu
$$
(so $\dot y(t)=f(y(t),u(t))$ for $t\geq 0$, with $y(0)=x$), and 
$$
  \ell(x,u) = \frac{1}{2} \<x, Q x\> + \frac{1}{2} \<u, R u\>.
$$
with $Q,R$ positive definite matrices.

The exact DPP is, for any $h>0$ and $x\in \R^d$:
$$
    v(x) = \inf_{u(.)\in \cU} \bigg( \int_0^h e^{-\ml t} \ell(y_x^u(t),u(t))dt + e^{-\ml h} v(y_x^a(h))\bigg)
$$
and the approximated DPP (the one we will use) will be of the form%
\footnote{with for instance $L(x,a)=h \ell(x,a)$ and $F(x,a)=x + h f(x,a)$ for a first order approximation,
or $L(x,a)= \frac{h}{2}(\ell(x,a) + e^{-\ml h}\ell(x+hf(x,a),a))$ and $F(x,a)=x + \frac{h}{2} (f(x,a) + f(x+hf(x,a),a))$
for a second order approximation.}
\be\label{eq:ex1-DPP-approx}
    V(x) = \inf_{a\in U} \big(L(x,a) + e^{-\ml h} V(F(x,a))\big).
\ee
\blue{
  Notations pour rester cohérent avec $F(x,a)=x+hf(x,a)$ 
  (donc avec "+", meme si dans le code actuel ce sera sans doute des "-"), et aussi cohérent avec ce qu'on a fait pour 
  le problème de max
\begin{itemize}
  \item Order=1 (Euler) : $ L(x,a)=  \ell(x,a) \dt$
  \item Order=2 (RK2) :  $ L(x,a)= e^{-\ml \dt/2}  \ell(x + \frac{\dt}{2} f(x,a),a) \dt$ ("point milieu")
    %\item RK 2-1 :  $L(x,a)=  \ell(x -0.5 h (F(x,a)+ F(x-h F(x,a),a)),a)  h $ ?
  \item Order=2.1 (RK2) : $L(x,a)=  \frac{\dt}{2} \big(\ell(x,a) +  e^{-\ml \dt}\ell (x+\dt f(x,a),a) \big)$ ("trapèze")
  \item Order=10 : $p$ fois la formule "2.1" précédente (avec $p\geq 1$)
    soit 
      %$$L(x,a)= h\sum_{k=0}^{p-1} e^{-\ml h(k+\frac{1}{2})} \ell(x+ h (k+\frac{1}{2}),\, a) $$
    $$L(x,a)= h\sum_{k=0}^{p} d_k e^{-\ml h k} \ell(x+ h k, a) $$ 
    où $h=\frac{\dt}{p}$ et $d_0=d_p=\small\frac{1}{2}$ et $d_k=1$ pour $1\leq k\leq p-1$.
    (On aurait pu prendre aussi $p$ fois la formule de point milieu précédente, ce qui donnerait
    $L(x,a)= h\sum_{k=0}^{p-1} e^{-\ml h (k+1/2)} \ell(x+ h (k+1/2), a) $.)
  \item Order=20 : arret avec message erreur (on pourrait faire des quadratures plus précises pour l'intégrale).
\end{itemize}
}
\red{
Pour l'ordre 10 pas plutôt
 $$L(x,a)= h\sum_{k=0}^{p} d_k e^{-\ml h k} \ell(x_k, a) $$ 
 avec $x_0=x$, $x_{k+1}= x_k + h f(x_k,a)$, $k=1,p$ ?\\
}
The corresponding HJB equation is 
\be\label{eq:ex1-hjb}
  \ml v(x) + \max_{u\in U} (-f(x,u) \cdot \nabla V(x) - \ell(x,u))=0, \quad x\in \R^d.
\ee

Assuming some technical (controllability) conditions on $A,B$ we have an exact solution in the form
$v(x)= \frac{1}{2} \<x,Px\>$
where $P$ is a symmetric matrix of $\R^d$ which is the solution of the following Riccati equation:
$$ 0 = - \lambda P  + A^T P + P A - P C P + Q 
$$
where $C:=B R^{-1} B^T$.

Furthermore if we work in a finite box domain $x\in [-\bX,\bX]^d$ the optimal control $u(x)$ (in feedback form) 
can be bounded a priori, since here the exact solution is $u(x) = - R^{-1} B^T \nabla V(x) = R^{-1} B^T P x$.
So it suffices to consider that $u\in [-\bU,\bU]^q$ with $\bU := \|R^{-1} B^T P \|_\infty \bX$ 
in order to reach the maximum in
\eqref{eq:ex1-DPP-approx} or in  \eqref{eq:ex1-hjb}.

Example in dimension $d=2$: voir fichier \verb"test1.m"




